Mobile authentication of copy detection patterns

In the recent years, the copy detection patterns (CDP) attracted a lot of attention as a link between the physical and digital worlds, which is of great interest for the internet of things and brand protection applications. However, the security of CDP in terms of their reproducibility by unauthorized parties or clonability remains largely unexplored. In this respect this paper addresses a problem of anti-counterfeiting of physical objects and aims at investigating the authentication aspects and the resistances to illegal copying of the modern CDP from machine learning perspectives. A special attention is paid to a reliable authentication under the real life verification conditions when the codes are printed on an industrial printer and enrolled via modern mobile phones under regular light conditions. The theoretical and empirical investigation of authentication aspects of CDP is performed with respect to four types of copy fakes from the point of view of (i) multi-class supervised classification as a baseline approach and (ii) one-class classification as a real-life application case. The obtained results show that the modern machine-learning approaches and the technical capacities of modern mobile phones allow to reliably authenticate CDP on end-user mobile phones under the considered classes of fakes.

==> appendices/decomposition_tricks.tex <==
% ----------------------------------------
\section{Mutual information decomposition tricks}
\label{app:mutual info decomposition tricks}

According to the definition (\ref{ib-sup second term direct decomposition}) in Section \ref{subsubsec: sup class second term}, the mutual information  $I(\A; \C)$ can be decomposed as:
\begin{equation}
\begin{aligned} 
	I(\A; \C) & = \mathbb{E}_{\pac}  \left[  \log \frac{p(\c| \a)}{p(\c)}  \right] \\
              & = - \mathbb{E}_{p(\c)}  \left[  \log p(\c)\right] + \mathbb{E}_{\pac}  \left[  \log p(\c| \a)\right].
 \end{aligned} 
\label{ib-occ second term direct decomposition app}
\end{equation}
%
The first term of this decomposition corresponds to the entropy of class labels $H(\C) =\;$ $- \mathbb{E}_{p(\c)}  \left[ \log p(\c) \right]$. In the second term the transition probability $p(\c| \a)$ is unknown. At the same time, it can be written as:
%
\begin{equation}
\begin{aligned} 
\mathbb{E}_{\pac} \left[ \log p(\c|\a)\right] & =   \int_{\c}\int_{\a}  p(\a, \c)   \log p(\c|\a)   \ d\c \ d\a.
\end{aligned} 
\label{MI_2nd_unsupervised_cond_entropy1} 
\end{equation}
%
The expectation with respect to the joint distribution $\pac$ can also be defined via the marginalization $\pac = \int_{\x} p(\x,\a,\c)d\x = \int_{\x} p(\c, \x)q_{\bphi}(\a|\x) d\x$. Combing these results, one can obtain:    
%
%
%\begin{equation}
\begin{multline}
    \mathbb{E}_{p(\a,\c)}  \left[  \log p(\c| \a)\right] =  \\
    %
    = \int_{\c}\int_{\a}\int_{\x}  p(\c,\x) q_{\bphi}(\a|\x)  \log p(\c|\a) \ d\c  \ d\a \ d\x \\ 
    %
    = \mathbb{E}_{p(\c, \x)}  \left[   \mathbb{E}_{q_{\bphi}(\a|\x)} \left[  \log p(\c| \a) \right]\right].
\label{MI_2nd_unsupervised_cond_entropy2}    
\end{multline}
%\label{MI_2nd_unsupervised_cond_entropy2}
%\end{equation}
%
%
To overcome the problem of unknown $p(\c| \a)$, a variational distribution $p_{\btheta}(\c| \a)$ parametrized via a set of parameters $\btheta$ is applied to approximate $p(\c| \a)$:
%
\begin{equation}
 \begin{aligned} 
\label{MI_2nd_unsupervised_cond_entropy3}
    \mathbb{E}_{p(\a,\c)}  \left[  \log p(\c| \a)\right]  
    & =   \mathbb{E}_{p(\c,{\bf x} )}  \left[   \mathbb{E}_{q_{\bphi}(\a|{\bf x})} \left[  \log p(\c| \a) \frac{ p_{\btheta}(\c| \a)}{p_{\btheta}(\c| \a)} \right]\right] \\ 
    %
    & = \mathbb{E}_{p(\c,{\bf x} )}  \left[   \mathbb{E}_{q_{\bphi}(\a|{\bf x})} \left[  \log p_{\btheta}(\c| \a) \right]\right] \\
    %
    & \;\;\; + \mathbb{E}_{p(\a,\c)}  \left[ \log  \frac{p(\c| \a)}{p_{\btheta}(\c| \a)} \right],
 \end{aligned}
\end{equation}
%
where in the second term the expectation defined in (\ref{MI_2nd_unsupervised_cond_entropy2}) is used. 
%
%\begin{equation}
\begin{multline} 
    \mathbb{E}_{p(\a,\c )}  \left[ \log  \frac{p(\c| \a)}{p_{\btheta}(\c| \a)} \right] = \mathbb{E}_{p(\a )} \left[  \mathbb{E}_{p(\c|\a )}   \left[ \log  \frac{p(\c| \a)}{p_{\btheta}(\c| \a)} \right]\right] \\ 
    %
    =  \mathbb{E}_{p(\a)} \left[D_{\mathrm{KL}}\left(p(\c|\A=\a) \| p_{\btheta}(\c|\A=\a)\right)  \right] \\ 
    %
    = D_{\mathrm{KL}}\left(p(\c|\a ) \| p_{\btheta}(\c|\a)\right).
\label{MI_2nd_unsupervised_cond_entropy4}
\end{multline} 
%\end{equation}
%
%
Since the KL-divergence $D_{\mathrm{KL}}\left(p(\c|\a ) \| p_{\btheta}(\c|\a)\right) \geq 0$, the (\ref{MI_2nd_unsupervised_cond_entropy3}) can be lower bounded as:
%
\begin{equation}
\begin{aligned}
\mathbb{E}_{p(\a,\c)}  \left[  \log p(\c| \a)\right]  & \geq \mathbb{E}_{p(\c,\x )}  \left[ \mathbb{E}_{q_{\bphi}(\a|\x)} \left[  \log p_{\btheta}(\c| \a) \right]\right].
\end{aligned}
\label{MI_2nd_unsupervised_cond_entropy5}
\end{equation}
%
%
Therefore, the mutual information (\ref{ib-occ second term direct decomposition app}) can be lower bounded as  $I(\A; \C) \geq I_{\btheta, \bphi_\rma}(\A;\C)$, where the lower bound is defined as:
%
\begin{equation}
\begin{aligned} 
    I_{\btheta, \bphi_\rma}(\A;\C) & \triangleq H(\C) + \mathbb{E}_{p(\c,\x )}  \left[   \mathbb{E}_{q_{\bphi}(\a|\x)} \left[  \log p_{\btheta}(\c| \a) \right]\right]
 \\ & = H(\C) - H_{\btheta, \bphi_\rma} (\C|\A),
\end{aligned} 
\label{IB_S_lower_bound1}
\end{equation}
%
where $H_{\btheta, \bphi_\rma} (\C|\A) = - \mathbb{E}_{p(\c,\x )}  \left[\mathbb{E}_{q_{\bphi}(\a|\x)} \left[  \log p_{\btheta}(\c| \a) \right]\right]$.


==> appendices/spatial_domain.tex <==
\section{Spatial domain analysis}
\label{app:spatial domain analysis}

%--- One metric digital vs physical ---------------------------
\begin{figure}[h!]
	\centering
	%
	\begin{subfigure}{0.48\columnwidth}
		\centering
		\captionsetup{justification=centering}
        \includegraphics[width=1\linewidth,valign=t]{appendices/spatial_domain/one_metrics/rgb_pearson_330_x_330_normalised.png}
	    \caption{Pearson correlation with respect to \\ the digital templates/references.}
	    \label{fig:spatial domain digital pearson gray main}
	\end{subfigure}		
	%
	%%\hspace{0.2cm}
	%
	\begin{subfigure}{0.48\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=1\linewidth,valign=t]{appendices/spatial_domain/one_metrics/rgb_phisical_references_pearson_330_x_330_normalised.png}
	    \caption{Pearson correlation with respect to \\the physical references.}
	    \label{fig:spatial domain physical pearson rgb main}
	\end{subfigure}		
	%
	\\ [1cm]
	%
	\begin{subfigure}{0.48\columnwidth}
		\centering
		\captionsetup{justification=centering}
        \includegraphics[width=1\linewidth,valign=t]{appendices/spatial_domain/one_metrics/rgb_xor_otsu_330_x_330_normalised.png}
	    \caption{Hamming distance with respect to \\ the digital templates/references.}
	    \label{fig:spatial domain digital xor otsu gray main}
	\end{subfigure}		
	%
	%%\hspace{0.2cm}
	%
	\begin{subfigure}{0.48\columnwidth}
		\centering
		\captionsetup{justification=centering}
        \includegraphics[width=1\linewidth,valign=t]{appendices/spatial_domain/one_metrics/rgb_phisical_references_xor_otsu_330_x_330_normalised.png}
	    \caption{Hamming distance with respect to \\ the binarized physical references.}
	    \label{fig:spatial domain physical xor otsu rgb main}
	\end{subfigure}		
	%
	\\ [1cm]
	%
    \caption{The distribution of the Hamming  distances between the references (digital or physical) and the corresponding printed codes (original and fakes). In case of the physical references the binarization is applied as a simple thresholding with an optimal threshold determined individually for each code via Otsu's method.}
    \label{fig:spatial domain digital vs physical one metric main}        
\end{figure}

%------------------------------

%--- One meteric 1 ---------------------------
\begin{figure}[h!]
	\centering
	
	\begin{subfigure}{0.48\columnwidth}
		\centering
		\captionsetup{justification=centering}
        \includegraphics[width=1\linewidth,valign=t]{appendices/spatial_domain/one_metrics/rgb_l1_330_x_330_normalised.png}
	    \caption{$\ell_1$ distance with respect to \\ the digital templates/references.}
	    \label{fig:spatial domain digital l1 rgb}
	\end{subfigure}		
	%
	%\hspace{0.2cm}
	%
	\begin{subfigure}{0.48\columnwidth}
		\centering
		\captionsetup{justification=centering}
        \includegraphics[width=1\linewidth,valign=t]{appendices/spatial_domain/one_metrics/rgb_phisical_references_l1_330_x_330_normalised.png}
	    \caption{$\ell_1$ distance with respect to \\ the physical reference.}
	    \label{fig:spatial domain physical l1 rgb}
	\end{subfigure}	
	%
	\\ [0.6cm]
	%
	\begin{subfigure}{0.48\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=1\linewidth,valign=t]{appendices/spatial_domain/one_metrics/rgb_mse_330_x_330_normalised.png}
	    \caption{$\ell_2$ distance with respect to \\ the digital templates/references.}
	    \label{fig:spatial domain digital l2 rgb}
	\end{subfigure}		
	%
	%\hspace{0.2cm}
	%
	\begin{subfigure}{0.48\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=1\linewidth,valign=t]{appendices/spatial_domain/one_metrics/rgb_phisical_references_l1_330_x_330_normalised.png}
	    \caption{$\ell_2$ distance with respect to \\ the physical reference.}
	    \label{fig:spatial domain physical l2 rgb}
	\end{subfigure}		
	%
	\\ [0.6cm]
	%
    \caption{The distribution of the $\ell_1$ and $\ell_2$ distances between the references (digital or physical) and the corresponding printed codes (original and fakes).}
    \label{fig:spatial domain digital l1 l2 metric digital vs physical}        
\end{figure}

%------------------------------

%--- Two metric 1 ---------------------------
\begin{figure}[h!]
	\centering
	%
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=0.975\linewidth,valign=t]{appendices/spatial_domain/two_metric/binary_reference_rgb_l1_vs_xor_otsu.png}
	    \caption{$\ell_1$ vs Hamming distance with respect \\ to the digital templates/references.}
	    \label{fig:spatial domain gray l1 vs xor otsu digital}
	\end{subfigure}		
	%
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=0.975\linewidth,valign=t]{appendices/spatial_domain/two_metric/physical_reference_rgb_l1_vs_xor_otsu.png}
	    \caption{$\ell_1$ vs Hamming distance with respect \\ to the physical references.}
	    \label{fig:spatial domain rgb l1 vs xor otsu physical}
	\end{subfigure}		
	%
	\\ % --- raw 2 ----
	%
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=0.975\linewidth,valign=t]{appendices/spatial_domain/two_metric/binary_reference_rgb_mse_vs_l1.png}
	    \caption{$\ell_2$ vs $\ell_1$ distances with respect \\ to the digital templates/references.}
	    \label{fig:spatial domain gray l1 vs l2 digital}
	\end{subfigure}		
	%
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=0.975\linewidth,valign=t]{appendices/spatial_domain/two_metric/physical_reference_rgb_mse_vs_l1.png}
	    \caption{$\ell_2$ vs $\ell_1$ distances with respect \\ to the physical references.}
	    \label{fig:spatial domain rgb l1 vs l2 physical}
	\end{subfigure}		
	%
	\\ % --- raw 3 ----
	%
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=0.975\linewidth,valign=t]{appendices/spatial_domain/two_metric/binary_reference_rgb_mse_vs_xor_otsu.png}
	    \caption{$\ell_2$ vs Hamming distance with respect \\ to the digital templates/references.}
	    \label{fig:spatial domain gray l2 vs xor otsu digital}
	\end{subfigure}		
	%
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=0.975\linewidth,valign=t]{appendices/spatial_domain/two_metric/physical_reference_rgb_mse_vs_xor_otsu.png}
	    \caption{$\ell_2$ vs Hamming distance with respect \\ to the physical references.}
	    \label{fig:spatial domain rgb l2 vs xor otsu physical}
	\end{subfigure}		
	%
	\\
	%
    \caption{The 2D PGC separability in the spatial domain with respect to the $\ell_2$, $\ell_1$ and Hamming distances between the references (digital or physical) and the corresponding printed codes (original and fakes) (part 1).}
    \label{fig:spatial domain two metric part 1}        
\end{figure}

%------------------------------
%--- Two metric 2 ---------------------------
\begin{figure}[h!]
	\centering
	%
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=0.975\linewidth,valign=t]{appendices/spatial_domain/two_metric/binary_reference_rgb_pearson_vs_l1.png}
	    \caption{Pearson correlation vs $\ell_1$ distance with \\ respect to the digital templates/references.}
	    \label{fig:spatial domain gray pearson vs l1 digital}
	\end{subfigure}		
	%
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=0.975\linewidth,valign=t]{appendices/spatial_domain/two_metric/physical_reference_rgb_pearson_vs_l1.png}
	    \caption{Pearson correlation vs $\ell_1$ distance with \\ respect to the physical references.}
	    \label{fig:spatial domain rgb pearson vs l1 physical}
	\end{subfigure}		
	%
	\\ % --- raw 2 ----
	%
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=0.975\linewidth,valign=t]{appendices/spatial_domain/two_metric/binary_reference_rgb_pearson_vs_mse.png}
	    \caption{Pearson correlation vs $\ell_2$ distance with \\ respect to the digital templates/references.}
	    \label{fig:spatial domain gray pearson vs l2 digital}
	\end{subfigure}		
	%
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=0.975\linewidth,valign=t]{appendices/spatial_domain/two_metric/physical_reference_rgb_pearson_vs_mse.png}
	    \caption{Pearson correlation vs $\ell_2$ distance with \\ respect to the physical references.}
	    \label{fig:spatial domain rgb pearson vs l2 physical}
	\end{subfigure}		
	%
	\\ % --- raw 3 ----
	%
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=0.975\linewidth,valign=t]{appendices/spatial_domain/two_metric/binary_reference_rgb_pearson_vs_xor_otsu.png}
	    \caption{Pearson correlation vs Hamming distance \\ with respect to the digital templates/references.}
	    \label{fig:spatial domain gray pearson vs xor otsu digital}
	\end{subfigure}		
	%
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\captionsetup{justification=centering}		
        \includegraphics[width=0.975\linewidth,valign=t]{appendices/spatial_domain/two_metric/physical_reference_rgb_pearson_vs_xor_otsu.png}
	    \caption{Pearson correlation vs Hamming distance \\ with respect to the physical references.}
	    \label{fig:spatial domain rgb pearson vs xor otsu physical}
	\end{subfigure}		
	%
	\\
	%
    \caption{The 2D PGC separability in spatial domain with respect to the $\ell_2$, $\ell_1$, Hamming distances and Pearson correlation between the references (digital or physical) and the corresponding printed codes (original and fakes) (part 2).}
    \label{fig:spatial domain two metric part 2}        
\end{figure}

% ---------------------------------

==> datasets_table.tex <==
% -------------------------
\begin{table*}[t!]
	\centering
	\renewcommand*{\arraystretch}{1.5}
	%
	\caption{An overview of the datasets of CDP: the datasets (1) and (2) are publicly available state-of-the-art datasets and the dataset (3) is created and investigated in the current paper.}
	\label{tab:cdp datasets overview}
	{\small
	\begin{tabular}{l>{\centering\arraybackslash}m{0.15\linewidth}
	ccc>{\centering\arraybackslash}m{0.12\linewidth}} \hline
	 & Name & Digital templates & Printing & Acquisition & \# of codes \\ \hline
     %
     % DP1C \& DP1E
     %
	(1) & DP1C \& DP1E \cite{Taran2020icassp} & \multicolumn{1}{m{0.15\linewidth}}{ 
            \begin{itemize}[leftmargin=0cm,noitemsep,topsep=0pt]
                \item[] size: $384 \times 384$
                \item[] symbol size: $6 \times 6$                
            \end{itemize}  
            } 
		& \multicolumn{1}{m{0.2\linewidth}}{
			\textit{Laser}, at 1200 dpi: 
        	\begin{itemize}[leftmargin=0.2cm,noitemsep,topsep=0pt]
        		\item[] $\boldsymbol{\cdot}$ Samsung Xpress 430
	        	\item[] $\boldsymbol{\cdot}$ Lexmark CS310
    	    \end{itemize}
			\textit{Inkjet}, at 1200 dpi: 
        	\begin{itemize}[leftmargin=0.1cm,noitemsep,topsep=0pt]
                \item[] $\boldsymbol{\cdot}$ Canon PIXMA  iP7200
                \item[] $\boldsymbol{\cdot}$ HP OfficeJet Pro 8210
    	    \end{itemize}	    	    			
            } 
		& \multicolumn{1}{>{\centering\arraybackslash}m{0.18\linewidth}}{ 
            \begin{itemize}[leftmargin=0.2cm,noitemsep,topsep=0pt]
            	\item[] \textit{Scanner}:            
                \item[] $\boldsymbol{\cdot}$ Canon 9000F 
                \item[] $\;\;$ at 1200 ppi
                \item[] $\boldsymbol{\cdot}$ Epson V850 Pro
                \item[] $\;\;$ at 1200 ppi
            \end{itemize}  
            }  
%		& \multicolumn{1}{>{\centering\arraybackslash}m{0.123\linewidth}}{ 
%            \begin{itemize}[leftmargin=0cm,noitemsep,topsep=0pt]
%                \item[] $\;\;\;\;$ 384 $\times$
%                \item[] 4 printers $\times$
%                \item[] 2 scanners = 
%                \item[] $\;\;\;\;$ 3072 
%            \end{itemize}  
%            }    
		& \multicolumn{1}{m{0.1\linewidth}}{ % Conclusions:
            \begin{itemize}[leftmargin=0cm,noitemsep,topsep=0pt]
                \item[] digital: 384
                \item[] original: 3072
                \item[] fakes: 3072
                \item[] total: 6528
            \end{itemize}  
            }  
     \\[-0.35cm] \hline  
    %
    % CSGC
    %
	 (2) & CSGC \cite{yadav2019estimation} & \multicolumn{1}{m{0.15\linewidth}}{ 
            \begin{itemize}[leftmargin=0cm,noitemsep,topsep=0pt]
                \item[] size: $100 \times 100$
                \item[] symbol size: $1 \times 1$
            \end{itemize}  
            }    
		& \multicolumn{1}{m{0.2\linewidth}}{
			\textit{Laser}, at 600 dpi: 
        	\begin{itemize}[leftmargin=0.2cm,noitemsep,topsep=0pt]
        		\item[] $\boldsymbol{\cdot}$ Xerox Phaser 6500
    	    \end{itemize}
            }    
		& \multicolumn{1}{>{\centering\arraybackslash}m{0.18\linewidth}}{ 
            \begin{itemize}[leftmargin=0.2cm,noitemsep,topsep=1pt]
            	\item[] \textit{Scanner}:            
                \item[] $\boldsymbol{\cdot}$ Epson V850 Pro
                \item[] $\;\;$ at 2400 ppi
                \item[] $\;\;$ at 4800 ppi
                \item[] $\;\;$ at 9600 ppi                                
            \end{itemize}  
            }  
%       	& No available
		& \multicolumn{1}{m{0.1\linewidth}}{ % Conclusions:
            \begin{itemize}[leftmargin=0cm,noitemsep,topsep=0pt]
                \item[] digital: 950
                \item[] original: 2850
                %\item[] fakes: 0
                \item[] total: 3800
            \end{itemize}  
            }                    
     \\[-0.35cm] \hline     
     %
     % Indigo mobile
     %
 	 (3) & Indigo mobile  & \multicolumn{1}{m{0.15\linewidth}}{ 
            \begin{itemize}[leftmargin=0cm,noitemsep,topsep=0pt]
                \item[] size: $330 \times 330$
                \item[] symbol size: $5 \times 5$                
            \end{itemize}  
            }  
		& \multicolumn{1}{m{0.2\linewidth}}{
			\textit{Industrial}, at 812 dpi: 
        	\begin{itemize}[leftmargin=0.2cm,noitemsep,topsep=0pt]
        		\item[] $\boldsymbol{\cdot}$ HP Indigo 5500 DS
    	    \end{itemize}
            } 
		& \multicolumn{1}{>{\centering\arraybackslash}m{0.18\linewidth}}{ 
            \begin{itemize}[leftmargin=0.2cm,noitemsep,topsep=0pt]
            	\item[] \textit{Mobile phone}:            
                \item[] $\boldsymbol{\cdot}$ iPhone XS 
                \item[] $\;\;$ auto settings
            \end{itemize}  
            }  
%		& \multicolumn{1}{>{\centering\arraybackslash}m{0.18\linewidth}}{ 
%            \begin{itemize}[leftmargin=0cm,noitemsep,topsep=0pt]
%                \item[] $\;\;\;\;$ 300 $\times$
%                \item[] 2 copy machines $\times$
%                \item[] 2 paper types $\times$                
%                \item[] 1 phone = 
%                \item[] $\;\;\;\;$ 1200 
%            \end{itemize}  
%            }    
		& \multicolumn{1}{m{0.1\linewidth}}{ % Conclusions:
            \begin{itemize}[leftmargin=0cm,noitemsep,topsep=3pt]
                \item[] digital: 300
                \item[] original: 300
                \item[] fakes: 1200
                \item[] total: 1800
            \end{itemize}  
            }  
     \\[-0.35cm] \hline
                   
	\end{tabular}
	}
\end{table*}
% -------------------------
